Consensus or Conflict? Fine-Grained Evaluation of Conflicting Answers in Question-Answering

Large Language Models (LLMs) have demonstrated strong performance in question answering (QA) tasks. However, Multi-Answer Question Answering (MAQA), where a question may have several valid answers, remains challenging. Traditional QA settings often assume consistency across evidences, but MAQA can involve conflicting answers. Constructing datasets that reflect such conflicts is costly and labor-intensive, while existing benchmarks often rely on synthetic data, restrict the task to yes/no questions, or apply unverified automated annotation. To advance research in this area, we extend the conflict-aware MAQA setting to require models not only to identify all valid answers, but also to detect specific conflicting answer pairs, if any. To support this task, we introduce a novel cost-effective methodology for leveraging fact-checking datasets to construct NATCONFQA, a new benchmark for realistic, conflict-aware MAQA, enriched with detailed conflict labels, for all answer pairs. We evaluate eight high-end LLMs on NATCONFQA, revealing their fragility in handling various types of conflicts and the flawed strategies they employ to resolve them.

==> Figures/error_real_mistakes_examples.tex <==
\begin{table*}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} llp{3.5cm}p{4.5cm}p{2.5cm}l @{}}
\toprule
Model     & Category & Q-Type       & Question                                                                    & Model Output                                                                                             & Ref. Answers  & Error Type            \\ \midrule
c         & Normal   & boolean      & Are cities getting cooler compared to their surrounding areas?             & Studies show that, overall, urban and rural temperature trends are almost identical (so cities are not systematically cooling), yet about 42\% of monitored cities have actually become cooler than their surrounding rural areas.             & True, False   & conflict resolution    \\
GPT-4o    & Normal   & boolean      & Did the ice thickness decrease by 1 cm per year until 2007?                  & The passages do not provide a direct answer to whether the ice thickness decreased by 1 cm per year until 2007, but they indicate that the Greenland ice sheet experienced accelerating mass loss and thinning, particularly near the coasts, with significant ice loss reported in 2007. & True, False   & no\_answer             \\
o3-high   & Normal   & wh-function  & What was the hottest month recorded on Earth?                               & The passages identify three different months as holding the global heat record: June 2014, July 2015 and June 2019.                                                                                                                              & –             & over-generalization    \\
\bottomrule
\end{tabular}
\caption{Examples of model outputs on conflicting-answer questions, with annotated error types.}
\label{tab:sample-errors}
\end{table*}

